Adversarial Circuit Evaluation

Circuits are supposed to accurately describe how a neural network performs a specific task, but do they really? We evaluate three circuits found in the literature (IOI, greater-than, and docstring) in an adversarial manner, considering inputs where the circuit's behavior maximally diverges from the full model. Concretely, we measure the KL divergence between the full model's output and the circuit's output, calculated through resample ablation, and we analyze the worst-performing inputs. Our results show that the circuits for the IOI and docstring tasks fail to behave similarly to the full model even on completely benign inputs from the original task, indicating that more robust circuits are needed for safety-critical applications.

==> docstring-outputtable-original.tex <==
\begin{tblr}{X[l] X[l] c | c c c | c c c}
\toprule
input & patch input & loss & model 0 & model 1 & model 2 & circuit 0 & circuit 1 & circuit 2 \\
\midrule
\texttt{
def port(self, order, match, fields, model, old, parent):\newlinesymbol
    """agent rule manager\newlinesymbol
\newlinesymbol
    :param fields: set song\newlinesymbol
    :param model: plane action\newlinesymbol
:param} & <|BOS|>
def image(self, key, file, filename, files, line, expected):
    """package crime framework

    :param host: dollar author
    :param command: cup spring
    :param & 12.07 & \shortstack{' old'\\ (19.66)} & \shortstack{' new'\\ (17.75)} & \shortstack{' fields'\\ (16.64)} & \shortstack{' file'\\ (18.87)} & \shortstack{' filename'\\ (17.41)} & \shortstack{' line'\\ (16.74)} \\
<|BOS|>
def default(self, node, user, current, text, port, item):
    """export manager mission

    :param current: song spot
    :param text: delay draft
    :param & <|BOS|>
def model(self, shape, message, group, file, result, fields):
    """content host bed

    :param new: share stage
    :param page: lift range
    :param & 12.07 & \shortstack{' port'\\ (20.52)} & \shortstack{' current'\\ (15.69)} & \shortstack{' str'\\ (15.31)} & \shortstack{' port'\\ (17.82)} & \shortstack{' filename'\\ (17.39)} & \shortstack{' message'\\ (17.22)} \\
<|BOS|>
def default(self, node, user, current, text, port, item):
    """export manager mission

    :param current: song spot
    :param text: delay draft
    :param & <|BOS|>
def image(self, key, file, filename, files, line, expected):
    """package crime framework

    :param host: dollar author
    :param command: cup spring
    :param & 12.06 & \shortstack{' port'\\ (20.52)} & \shortstack{' current'\\ (15.69)} & \shortstack{' str'\\ (15.31)} & \shortstack{' file'\\ (19.44)} & \shortstack{' filename'\\ (17.97)} & \shortstack{' line'\\ (17.93)} \\
<|BOS|>
def create(self, token, field, request, content, order, new):
    """tree cut hell

    :param request: king bar
    :param content: income creation
    :param & <|BOS|>
def image(self, key, file, filename, files, line, expected):
    """package crime framework

    :param host: dollar author
    :param command: cup spring
    :param & 11.95 & \shortstack{' order'\\ (20.48)} & \shortstack{' request'\\ (18.78)} & \shortstack{' field'\\ (16.64)} & \shortstack{' file'\\ (20.19)} & \shortstack{' filename'\\ (17.68)} & \shortstack{' line'\\ (17.47)} \\
<|BOS|>
def values(self, json, module, count, end, model, index):
    """lead respect dust

    :param count: hell step
    :param end: volume pair
    :param & <|BOS|>
def image(self, key, file, filename, files, line, expected):
    """package crime framework

    :param host: dollar author
    :param command: cup spring
    :param & 11.90 & \shortstack{' model'\\ (21.46)} & \shortstack{' models'\\ (16.23)} & \shortstack{' id'\\ (15.41)} & \shortstack{' file'\\ (20.41)} & \shortstack{' filename'\\ (18.51)} & \shortstack{' line'\\ (17.95)} \\
<|BOS|>
def match(self, results, default, order, check, row, field):
    """activity path strength

    :param order: product plane
    :param check: fan bell
    :param & <|BOS|>
def image(self, key, file, filename, files, line, expected):
    """package crime framework

    :param host: dollar author
    :param command: cup spring
    :param & 11.88 & \shortstack{' row'\\ (20.65)} & \shortstack{' check'\\ (16.86)} & \shortstack{' bool'\\ (16.57)} & \shortstack{' file'\\ (19.56)} & \shortstack{' check'\\ (19.51)} & \shortstack{' line'\\ (18.09)} \\
<|BOS|>
def command(self, code, instance, create, size, sub, run):
    """border horse trip

    :param create: bishop attack
    :param size: duty horse
    :param & <|BOS|>
def image(self, key, file, filename, files, line, expected):
    """package crime framework

    :param host: dollar author
    :param command: cup spring
    :param & 11.80 & \shortstack{' sub'\\ (20.32)} & \shortstack{' run'\\ (15.97)} & \shortstack{' name'\\ (15.80)} & \shortstack{' file'\\ (20.00)} & \shortstack{' bool'\\ (17.52)} & \shortstack{' filename'\\ (17.31)} \\
<|BOS|>
def default(self, node, user, current, text, port, item):
    """export manager mission

    :param current: song spot
    :param text: delay draft
    :param & <|BOS|>
def error(self, order, shape, match, filename, message, results):
    """star opening risk

    :param file: cycle second
    :param content: race staff
    :param & 11.53 & \shortstack{' port'\\ (20.52)} & \shortstack{' current'\\ (15.69)} & \shortstack{' str'\\ (15.31)} & \shortstack{' item'\\ (18.44)} & \shortstack{' text'\\ (18.06)} & \shortstack{' int'\\ (17.22)} \\
<|BOS|>
def item(self, old, code, header, response, node, sub):
    """game phase birth

    :param header: cap session
    :param response: break player
    :param & <|BOS|>
def image(self, key, file, filename, files, line, expected):
    """package crime framework

    :param host: dollar author
    :param command: cup spring
    :param & 11.44 & \shortstack{' node'\\ (21.31)} & \shortstack{' code'\\ (17.17)} & \shortstack{' child'\\ (15.85)} & \shortstack{' file'\\ (20.06)} & \shortstack{' line'\\ (18.03)} & \shortstack{' node'\\ (17.91)} \\
<|BOS|>
def expected(self, root, results, host, module, names, files):
    """horse boot sector

    :param host: thinking rock
    :param module: rent tie
    :param & <|BOS|>
def error(self, action, image, source, old, text, content):
    """charge conduct wife

    :param task: meaning shadow
    :param field: warning self
    :param & 11.41 & \shortstack{' names'\\ (21.83)} & \shortstack{' name'\\ (19.86)} & \shortstack{' files'\\ (17.22)} & \shortstack{' image'\\ (17.93)} & \shortstack{' file'\\ (17.43)} & \shortstack{' name'\\ (17.00)} \\
\bottomrule
\end{tblr}


==> percentiles-paired-patches.tex <==
\begin{tblr}{lrrrrrr}
\toprule
   & \SetCell[c=2]{c} docstring  & & \SetCell[c=2]{c} greaterthan & & \SetCell[c=2]{c}{ioi} \\
 & \centering abs & \centering z-score & \centering abs & \centering z-score & \centering abs & \centering z-score \\
\midrule
count & 1000000.00 &  & 1000000.00 &  & 1000000.00 &  \\
mean & 1.38 &  & 0.08 &  & 0.59 &  \\
std & 0.93 &  & 0.06 &  & 0.53 &  \\
min & 0.01 & -1.46 & 0.01 & -1.29 & 0.00 & -1.10 \\
25\% & 0.71 & -0.72 & 0.04 & -0.66 & 0.21 & -0.71 \\
50\% & 1.11 & -0.28 & 0.07 & -0.25 & 0.42 & -0.32 \\
75\% & 1.78 & 0.43 & 0.10 & 0.32 & 0.80 & 0.39 \\
95\% & 3.29 & 2.04 & 0.20 & 1.94 & 1.65 & 1.98 \\
99\% & 4.57 & 3.41 & 0.33 & 3.99 & 2.49 & 3.57 \\
99.9\% & 6.06 & 5.01 & 0.46 & 6.14 & 3.85 & 6.12 \\
99.99\% & 7.33 & 6.37 & 0.54 & 7.45 & 5.34 & 8.92 \\
max & 9.97 & 9.19 & 0.60 & 8.47 & 8.83 & 15.47 \\
\bottomrule
\end{tblr}

